Accessibility for Whom? Perceptions of Sidewalk Barriers Across Disability Groups and Implications for Designing Personalized Maps

Despite diverse mobility needs worldwide, existing mapping tools fail to address the varied experiences of different mobility device users. This paper presents a large-scale online survey exploring how five mobility groups -- users of canes, walkers, mobility scooters, manual wheelchairs, and motorized wheelchairs -- perceive sidewalk barriers. Using 52 sidewalk barrier images, respondents evaluated their confidence in navigating each scenario. Our findings (N=190) reveal variations in barrier perceptions across groups, while also identifying shared concerns. To further demonstrate the value of this data, we showcase its use in two custom prototypes: a visual analytics tool and a personalized routing tool. Our survey findings and open dataset advance work in accessibility-focused maps, routing algorithms, and urban planning.

==> tables/ranking-comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\small
\centering
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{@{}lrrrrrr@{}}
\begin{tabular}{@{}l p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} @{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\textbf{Sidewalk barriers} &
 \cellcolor[HTML]{FFFFFF}\textbf{Walking Cane} &
 \cellcolor[HTML]{FFFFFF}\textbf{Walker} &
 \cellcolor[HTML]{FFFFFF}\textbf{Mobility Scooter} &
 \cellcolor[HTML]{FFFFFF}\textbf{Manual Whlchair} &
 \cellcolor[HTML]{FFFFFF}\textbf{Power Whlchair} &
 \cellcolor[HTML]{FFFFFF}\textbf{Avg Rank} \\
\midrule
\cellcolor[HTML]{FFFFFF}Missing curb ramps &
  \cellcolor[HTML]{F4D9E1}4.38 &
  \cellcolor[HTML]{DC86A1}1.56 &
  \cellcolor[HTML]{DD8BA5}1.71 &
  \cellcolor[HTML]{E3A0B5}2.45 &
  \cellcolor[HTML]{DE8DA6}1.79 &
  \cellcolor[HTML]{FFFF00}2.38 \\
 
\cellcolor[HTML]{F3F3F3}Uneven sidewalk panels &
  \cellcolor[HTML]{E197AE}2.13 &
  \cellcolor[HTML]{E29DB2}2.32 &
  \cellcolor[HTML]{E6ABBE}2.81 &
  \cellcolor[HTML]{D6EFE6}6.57 &
  \cellcolor[HTML]{DF93AB}1.99 &
  \cellcolor[HTML]{FFFF00}3.16 \\

\cellcolor[HTML]{F3F3F3}Steep sidewalk &
  \cellcolor[HTML]{DC88A3}1.63 &
  \cellcolor[HTML]{F7E4EA}4.75 &
  \cellcolor[HTML]{FBFEFD}5.76 &
  \cellcolor[HTML]{ECC0CE}3.52 &
  \cellcolor[HTML]{FFFFFF}5.66 &
  \cellcolor[HTML]{FFFF00}4.26 \\ 
  
\cellcolor[HTML]{FFFFFF}Broken surface/cracks &
  \cellcolor[HTML]{E9B4C4}3.11 &
  \cellcolor[HTML]{DE8EA7}1.82 &
  \cellcolor[HTML]{F0CCD7}3.93 &
  \cellcolor[HTML]{BEE6D7}7.10 &
  \cellcolor[HTML]{EAF7F2}6.13 &
  \cellcolor[HTML]{FFFF00}4.42 \\
  
\cellcolor[HTML]{F3F3F3}Narrow sidewalk &
  \cellcolor[HTML]{F3D7DF}4.30 &
  \cellcolor[HTML]{E8B0C2}2.99 &
  \cellcolor[HTML]{FCFEFE}5.73 &
  \cellcolor[HTML]{FEFBFC}5.56 &
  \cellcolor[HTML]{F6E1E7}4.65 &
  \cellcolor[HTML]{FFFF00}4.65 \\

\cellcolor[HTML]{FFFFFF}Sand/gravel &
  \cellcolor[HTML]{EFC8D4}3.80 &
  \cellcolor[HTML]{F6E1E8}4.67 &
  \cellcolor[HTML]{D7EFE6}6.56 &
  \cellcolor[HTML]{F1D0DA}4.07 &
  \cellcolor[HTML]{D2EEE4}6.65 &
  \cellcolor[HTML]{FFFF00}5.15 \\

\cellcolor[HTML]{F3F3F3}Grass surface &
  \cellcolor[HTML]{F0F9F6}6.00 &
  \cellcolor[HTML]{BBE5D6}7.15 &
  \cellcolor[HTML]{9ED9C3}7.80 &
  \cellcolor[HTML]{BDE5D6}7.12 &
  \cellcolor[HTML]{6FC6A6}8.84 &
  \cellcolor[HTML]{FFFF00}7.38 \\

\cellcolor[HTML]{FFFFFF}Brick/cobblestone &
  \cellcolor[HTML]{CCEBE0}6.78 &
  \cellcolor[HTML]{CDECE0}6.77 &
  \cellcolor[HTML]{69C4A2}8.97 &
  \cellcolor[HTML]{97D6BF}7.95 &
  \cellcolor[HTML]{98D7C0}7.93 &
  \cellcolor[HTML]{FFFF00}7.68 \\

\cellcolor[HTML]{F3F3F3}Manholes &
  \cellcolor[HTML]{B8E3D4}7.22 &
  \cellcolor[HTML]{AADECB}7.54 &
  \cellcolor[HTML]{83CFB3}8.38 &
  \cellcolor[HTML]{79CAAD}8.61 &
  \cellcolor[HTML]{C0E7D9}7.05 &
  \cellcolor[HTML]{FFFF00}7.76 \\
  
\bottomrule
\end{tabular}%
%}
\caption{The result of Survey Part 3: sidewalk barriers ranked per mobility group based on Kemeny-Young rank aggregation. The table is sorted by the average rank position across groups in decreasing order of perceived difficulty from most difficult barrier (top) to least (bottom). }
\label{tab:ranking-9-barriers}
\end{table}
